Q-learning-based Opportunistic Communication for Real-time Mobile Air Quality Monitoring Systems

We focus on real-time air quality monitoring systems that rely on devices installed on automobiles in this research. We investigate an opportunistic communication model in which devices can send the measured data directly to the air quality server through a 4G communication channel or via Wi-Fi to adjacent devices or the so-called Road Side Units deployed along the road. We aim to reduce 4G costs while assuring data latency, where the data latency is defined as the amount of time it takes for data to reach the server. We propose an offloading scheme that leverages Q-learning to accomplish the purpose. The experiment results show that our offloading method significantly cuts down around 40-50% of the 4G communication cost while keeping the latency of 99.5% packets smaller than the required threshold.

==> 1-introduction_old.tex <==
The development artificial intelligence in recent years prepares the ground for making IoT devices become smarter. IoT devices have ability to communicate and share information together, that help a wide range of processes, tasks can be solved quickly. For example, integrating sensors into a bus system in a city can monitor and provide detail information about air quality. However, those devices have low battery-capacity and also are costly for operation likes sending data to and receiving data from cloud server. One feasible solution is locating Road-Side-Units(RSUs) along roads, where buses operate in. RSUs are able to retrieve and process data from sensor with low-cost and high-reliability for transferring data. As a consequence, using connections between sensors to RSUs is more efficient than utilizing sensor-server connections.
% Với sự phát triển nhanh chóng của các thiết bị IoT và trí tuệ nhân tạo (AI) trong những năm gần đây đã xây dựng nền móng đầy hứa hẹn giúp các thiết bị IoT ngày càng trở lên thông minh hơn \cite{merenda2020edge}. Các thiết bị IoT có khả năng giao tiếp và chia sẻ thông tin với nhau, giúp cho nhiều quy trình, hoạt động, tác vụ trở nên thông minh hơn. Có thể kể tới những thiết bị Sensor được đặt trên xe bus trong thành phố có khả năng giám sát và cung cấp thông tin chi tiết về chất lượng không khí. Tuy nhiên, các thiết bị này có dung lượng thấp và tốn chi phí cho việc vận hành khi liên tục gửi và nhận dữ liệu với máy chủ Cloud. Một giải pháp cho vấn đề này là đặt các đơn vị điện toán biên (RSU) ở ven đường trên các tuyến đường có xe bus đi qua. Các thiết bị RSU này có khả năng tính toán và tiếp nhận thông tin từ các Sensor với chi phí truyền tin thấp và độ tin cậy truyền tin cao.  Kết quả là, việc sử dụng kết nối gửi dữ liệu thông qua các đơn vị RSU giúp giảm thiểu chi phí đáng kể so với truyền tin lên máy chủ Cloud.

In the other hand, a RSU has a small radius of connection range to sensors. Therefore, the network of RSUs does not have the ability to cover all connections in a city. Meanwhile, data collected by sensors needs to be sent to the Air Quality Server within a specific period of time. In order to solve this issue, we can combine two above-mentioned methods: the first one is sending data from a sensor to RSUs and the second one is to Cloud Server( named gNodeB-gNB) with a significant consideration about delay and cost of transferring data. We call this model three-tier network model including: sensors integrated in buses, RSUs and gNB, we also acknowledge that sensors are able to communicate themselves.
% Tuy nhiên, các đơn vị RSU có bán kính truyền tin tương đối nhỏ với các thiết bị cảm biến. Vì vậy mà mạng lưới các RSU chưa có khả năng bao phủ kết nối của toàn thành phố. Trong khi đó, thông tin thu thập được từ các Sensor cần được gửi về trung tâm quản lý chất lượng không khí (Air quality Server) trong một khoảng thời gian nhất định. Giải pháp cho vấn đề này là sử dụng kết hợp các phương thức truyền tin: gửi giữ liệu tới các đơn vị RSU hoặc gửi dữ liệu lên Cloud (gọi là gNodeB - gNB) sao cho đảm bảo thời gian trễ của gói tin với chi phí truyền tin thấp nhất.  Chúng tôi gọi mô hình truyền tin này là mô hình ba tầng bao gồm: các sensor được đăt trên xe bus, các thiết bị RSU, trung tâm xử lý GnB. Trong đó các sensor cũng có khả năng truyền tin cho nhau. 

In the last few years, scientists witnessed many AI-breakthroughs, which are applied in numerous areas, such as: natural language processing and image processing. However, using an AI model in a sensor with low battery capacity is practically hard but not impossible. With reinforcement learning (RL) methods, nowadays, we can build a lightweight model which could solve various kinds of uncertainty decision making problems. RL models are capable of continuously learning to modify its strategies which are adaptable to a fast changing environment. In our problem, as the environment keeps altering itself, each sensor is an agent with ability to make optimal decisions depends on the environment around. The main contributions of our work include:
% Gần đây, AI cũng có nhiều đột phá và được ứng dụng vào nhiều lĩnh vực khác nhau như: xử lý ngôn ngữ tự nhiên và nhận diện hình ảnh. Tuy nhiên, việc sử dụng các mô hình tính toán lớn là tương đối bất khả thi đối với các thiết bị Sensor vốn có dung lượng lưu trữ và tốc độ xử lý hạn chế. May mắn thay, là một phương pháp AI đầy hứa hẹn, học tăng cường có lợi thế rất lớn đối với các vấn đề đưa ra quyết định không chắc chắn với tốc độ xử lý nhanh chóng trên các thiết bị IoT nói chung. Các mô hình học tăng cường có khả năng học hỏi liên tục không ngừng nghỉ để cải thiện chiến lược của mình, đáp ứng được những thay đổi liên tục từ môi trường xung quanh. Do môi trường không ổn định nên trong nghiên cứu này, chúng tôi đề xuất mỗi thiết bị sensor là một tác nhân có khả năng đưa ra quyết định tối ưu tùy thuộc vào môi trường xung quanh của chính nó trên suốt tuyến đường xe bus cố định trong thành phố. Đóng góp chính trong nghiên cứu này của chúng tôi bao gồm:

\begin{itemize}
    \item Using RL method to optimize 2 tasks at the same time: delay and cost of sending infomation packets.
    \item Propose a model combining Fuzzy-logic and Q-learning in order to make optimal communication decisions. 
    \item Compare our result to other normal strategies in a simulator based on data of bus system of Seattle, Washington.
    \cite{jetcheva2003design}.
\end{itemize}
% \begin{itemize}
%     \item Sử dụng phương pháp học tăng cường nhằm tối ưu hóa cùng lúc 2 tác vụ: chi phí truyền tin và độ trễ của gói tin. 
%     \item Chúng tôi đề xuất sử dụng Fuzzy-logic kết hợp với Q-learning để tính toán đưa ra các quyết định truyền tin tối ưu. 
%     \item Đánh giá kết quả hiệu suất của thuật toán chúng tôi đề xuất với các phương pháp đưa ra quyết định thông thường bằng các giả lập dựa trên trên bộ dữ liệu về lộ trình xe bus của thành phố Seattle, Washington \cite{jetcheva2003design}.
% \end{itemize}

The remaining part of this paper is structured as follow: the second part is about related works; the third part describes the detail structure of our network model; the fourth part introduces a method which is the combination of Fuzzy-logic and Q-learning; The fifth part is about experiments and results; and the final part summarizes our work and proposes several further research directions.
% Phần còn lại của bài báo này được phân bổ như sau. Phần tiếp theo giới thiệu sơ lược về các công trình nghiên cứu liên quan. Phần \ref{sec:network_model} mô tả về kiến trúc mô hình của bài toán. Phần \ref{sec:fuzzy_q_learning}, chúng tôi đề xuất phương pháp kết hợp Fuzzy Logic với Q-Learning để điều chỉnh phần thưởng. Phần \ref{sec:experimental} bao gồm các kết quả thí nghiệm đánh giá hiệu suất của thuật toán. Cuối cùng, phần \ref{sec:conclusion_and_future_work} bao gồm tổng kết và các hướng phát triển tiếp theo.




==> 2-relatedwork.tex <==
% Vấn đề truyền tin của các Sensor đặt cố định trên xe Bus liên quan đến các nghiên cứu về điện toán biên (MEC), Reinforcement Learning và Fuzzy Logic.

Overview of transferring packages of sensors integrated in buses and problems related to Mobile Edge Computing(MEC), Reinforcement Learning and Fuzzy Logic.

\subsection{Mobile Edge Computing}
There are various research works based on MEC model. It is a very promising research direction attracting many researchers, for examples: a wide range of MEC applications can be found in \cite{xu2019blockchain}, \cite{zhang2018dual}. Authors in Ko et al. \cite{ko2018wireless} proposed a MEC model for large scale network and used random geometry in order to analyze the network delay. In \cite{2_tier_1} considers about sending packets problem and optimizing network resources distribution. Research of Zhao et al. \cite{3-tier_1} utilizes both MEC and MCC \nguyen{should define MCC} to send packets. Specifically, in this paper, sensors and devices are able to offload tasks to MEC server or Cloud server through RSUs with an objective that is maximizing system utilities by optimizing network resources distribution and the network strategy for offloading tasks.
% Trong những năm gần đây, có rất nhiều các công trình nghiên cứu dựa trên kiến trúc mô hình MEC. Đây là mô hình đầy hứa hẹn thu hút nhiều chú ý của các nhà nghiên cứu, có thể kể đến nhiều ứng dụng như trong  \cite{xu2019blockchain}, \cite{zhang2018dual}. Nghiên cứu của Ko et al. \cite{ko2018wireless} đề xuất mô hình MEC cho các mạng quy mô lớn và hình học ngẫu nhiên được sử dụng để phân tích độ trễ của mạng. Trong nghiên cứu của Feng et al. \cite{2_tier_1}, đã xem xét đến các vấn đề truyền tin và tối ưu hóa phân bổ tài nguyên. Hay trong nghiên cứu của Zhao et al. \cite{3-tier_1} đã đề xuất phương pháp sử dụng đồng thời MEC và MCC để truyền tin. Cụ thể, các thiết bị có thể tải các tác vụ tính toán lên máy chủ MEC hoặc máy chủ đám mây thông qua các RSU. Mục tiêu nhằm tối đa hóa tiện ích hệ thống bằng cách tối ưu hóa các chiến lược truyền tin và phân bổ tài nguyên.
In difference from previous studies, our paper based on three-tier network, provided various ways for offloading packets mentioned in \ref{sec:introduction}. Our target is to determine the optimal transmission way in order to minimizing cost and delay of packets generated by our network.
% Khác với các công trình nghiên cứu trước đây, bài báo chúng tôi nghiên cứu dựa trên mô hình ba tầng, cung cấp đa dạng các con đường truyền tin được đề cập trong \ref{sec:introduction}. Mục tiêu của chúng tôi là xác định đường truyền tối ưu để giảm thiểu chi phí truyền tin và độ trễ của các gói tin được sinh ra trong mạng.

\subsection{Reinforcement Learning}
% Reinforcement Learning (RL) đóng vai trò quan trọng trong các bài toán truyền tin trong MEC. Trong nghiên cứu của Gao et al. \cite{gao2020q} đã đề xuất chính sách quyết định truyền tin dựa trên giải thuật Q-learning để phân bổ và giảm tải tài nguyên tính toán. Cụ thể, nhóm tác giả mô tả quy trình quyết định truyền tin dưới dạng quy trình Markov và thiết kế hàm trạng thái cùng (state loss function (STLF)) để đánh giá mức độ tối ưu của hệ thống.
Reinforcement Learning always plays an essential role in communication problems in MEC. Gao et al. \cite{gao2020q} propose a method based on Q-learning aiming to distribute and offload computational resource. 
Specifically, they describe their strategy as a form of Markov process and also design a state loss function(STLF) in order to evaluate system's optimization.

% Tang et al. \cite{tang2020deep} propose a model-free deep reinforcement learning-based distributed algorithm, where each device can determine its offloading decision without knowing the task models and offloading decision of other devices. Để cải thiện ước tính chi phí dài hạn, nhóm tác giả đã kết hợp mô hình long short-term memory (LSTM), dueling deep Q-network (DQN), and double-DQN techniques trên các thiết bị có khả năng tính toán tương đối lớn.
Tang et al. \cite{tang2020deep} propose a model-free deep reinforcement learning-based distributed algorithm, where each device can determine its offloading decision without knowing the task models and offloading decision of other devices. In order to improve long-term cost estimation, these authors combine long short-term memory(LSTM), dueling deep Q-network(DQN), and double-DQN techiniques in devices with strong computing power. 

% Tuy nhiên, trong nghiên cứu của chúng tôi, những Sensor thu thập chất lượng không khí lại có khả năng tính toán tương đối hạn chế. Thay vì sử dụng các hệ thống mô hình lớn và phức tạp, chúng tôi mô tả mô hình dưới dạng quy trình Markov và sử dụng thuật toán Q-learning cùng các định nghĩa về hàm trạng thái và hàm phần thưởng để tối ưu.
In our research, sensors have weak computing power. Instead of using large and complicated model, we also use the combination of Markov chain and Q-learning with our design of state function and reward function for optimization.

\subsection{Fuzzy Logic}
% Fuzzy Logic đã được ứng dụng nhiều trong các lĩnh vực như xử lý tín hiệu \cite{reddy2019soft}, \cite{behera2018disease},  robot \cite{yang2018finite}, điều khiển thiết bị nhúng \cite{castillo2018generalized}. Trong MEC, Hossain et al. \cite{hossain2020fuzzy} đề xuất phương pháp sử dụng Fuzzy logic-based collaborative task offloading (FCTO) nhằm mục đích tối ưu chất lượng sử dụng dịch vụ của người dùng bằng cách giảm thiểu thời gian thực hiện các tác vụ. In FCTO, the delay sensitivity of the QoS is considered as the Fuzzy input parameter to make a decision where to offload the task is beneficial. The key is to share computation resources with each other and among MEC servers by using fuzzy-logic approach to select a target MEC server for task offloading. As a result, it can accommodate more computation workload in the MEC system and reduce reliance on the remote cloud. 
 
% Trong nghiên cứu này, chúng tôi đề xuất sử dụng Fuzzy Logic kết hợp với Q-learning để tối ưu phần thưởng và đưa ra các quyết định thông minh hơn. 
Fuzzy Logic is well-known for its applications in signal processing \cite{reddy2019soft}, \cite{behera2018disease},  robot \cite{yang2018finite}, controlling embedded devices \cite{castillo2018generalized}.
For applications in MEC, Hossain et al. \cite{hossain2020fuzzy} propose a method using Fuzzy logic-based collaborative task offloading (FCTO) with purpose of minimizing time for executing tasks. In FCTO, the delay sensitivity of the QoS is considered as the Fuzzy input parameter to make a decision where to offload the task is beneficial. The key is to share computation resources with each other and among MEC servers by using fuzzy-logic approach to select a target MEC server for task offloading. As a result, it can accommodate more computation workload in the MEC system and reduce reliance on the remote cloud.

In this paper, we suggest a model using Fuzzy-logic combined with Q-learning to make smarter decisions.


==> 3-systemmodel.tex <==
\subsection{Network Model} 
\begin{figure}
    \centering
    \includegraphics[width=8cm]{figs/model.eps}
    \caption{Network model}
    \label{fig:network_model}
\end{figure}
Figure \ref{fig:network_model} depicts the network model which comprises of three components: air quality monitoring devices, Road-Side-Units (RSUs), and a cloud server. 
We assume that there are $n$ air quality monitoring devices that are mounted on $n$ buses. 
Each device $S_i$ has a commuting capacity of $C_i$ and the transmission of $r_{S_i}$. 
The RSUs are computing units located along the roads. 
We also assume that there are $m$ RSUs denoted as $R_j (j = 1,...,m)$ which has the transmission radius of $r_{R_j}$.
The cloud server is named as the \emph{air quality server}.
There are three communication planes: 
\begin{itemize}
    \item Device 
\end{itemize}
Basically, there are 3 types of transmission line:
\begin{enumerate}
\item Sensor $\rightarrow$ gNB $\rightarrow$ Air quality server.
\item Sensor $\rightarrow$ RSU $\rightarrow$ Air quality server.
\item Sensor A $\rightarrow$ Sensor B.
\end{enumerate}
The connection are depicted as below (specifically in the table \ref{tab:params}):
\begin{itemize}
\item Sensor $\rightarrow$ gNB: wireless connection, very slow speed.
\item Sensor $\rightarrow$ RSU: wireless connection, slow speed. 
\item Sensor A $\rightarrow$ Sensor B: wireless connection, slow speed.
\item gNB $\rightarrow$ Air quality server: wired connection, fast speed.
\item RSU $\rightarrow$ Air quality server: wired connection, fast speed.
\end{itemize}
Sensor is able to transfer information packets to another Sensor or RSU even when they are within each other's coverage. Every Sensor can always send information to the gNB. Our target is that each sensor will consecutively track the air quality along the roads and send the data collected to the Air quality server via 1 of 3 transmission ways listed above. However, transmission method of Sensor $\rightarrow$ 
gNB will be much more expensive. Therefore, the problem need to be solved is that How to minimize the number of packets are sending to the gNB and the necessary time for the packets to be delivered to the sever do not exceed the level $\delta$ specified previously.

The important symbols in this paper are listed in the following table:
\begin{table}[tb]
    \centering
    \caption{Notions \label{tab:notions}}
    \begin{tabular}{|m{1cm}|m{6.5cm}|}
    \hline
         \textbf{Notion} & \textbf{Description} \\
         \hline
         n & Number of Sensor \\
         m & Number of RSU \\
         $S$ & Sensor $S = \{S_1,...,S_i,...,S_n\}$ \\
         $r_{S_i}$ & Transmission radius of Sensor $i$ \\ 
         $C^*$ & Maximum capacity of Sensor\\
         $c_t$ & Capacity at state $t$ of Sensor \\
         $R$ & RSU $R = \{R_1,...,R_j,...,R_m\}$ \\ 
         $r_{R_j}$ & Transmission radius of RSU $j$ \\
         $\delta$ & Maximum time of the information packet \\
         $\mathcal{T}$ & Time slots $\mathcal{T} = \{1,...,t,...,T\}$ \\
         $\mathcal{S}$ & State space of the network\\
         $s_i(t)$ & State at a time $t$ of sensor $i$\\
         $\mathcal{A}$ & Action space of the network\\
         $a_i(t)$ & Action at a time $t$ of sensor $i$\\ 
         $\mu_t$ & Time to generate information packet \\
         $\Delta_t$ & Time since generating information packet to the time $t$\\
         $\theta$ & Parameter decide reward\\
         \hline
    \end{tabular}
\end{table}



==> 3-systemmodel_old.tex <==
\subsection{Network Model} 
\begin{figure}
    \centering
    \includegraphics[width=8cm]{figs/model.eps}
    \caption{Network model}
    \label{fig:network_model}
\end{figure}
Our considered network is depicted in Fig.\ref{fig:network_model}.
The network comprises three components: air quality monitoring devices mounted on buses, Road-Side-Units (RSUs) that are computing units located along roads, and a cloud server. 
We assume that there are $n$ air quality monitoring devices placed on $n$ buses. 
Each device $S_i$ has a commuting capacity of $C_i$ and the transmission of $r_{S_i}$. 
We also assume that there are $m$ RSUs denoted as $R_j (j = 1,...,m)$ which has the transmission radius of $r_{R_j}$.
The cloud server is named as the \emph{air quality server}.



Our architectural model is depicted in Figure \ref{fig:network_model}. To be specific, our system is based on a 3-tier MEC model that includes: Sensors placed on each bus, Road-Side-Units (RSUs) and a Cloud Processing Center (called gNB). Firstly, about sensor devices, We assume that there are $n$ sensor $S_i (i = 1,...,n)$ placed on  $n$ fixed-route bus. Each sensor has maximum capacity is $C^*_i$ and transmission radius $r_{S_i}$. Secondly,  $m$  RSU $R_j (j = 1,...,m)$ which has transmission radius $r_{R_j}$ are fixedly placed along the roads. Thirdly, a huge gNB which has a wide coverage area overlay to all Sensors. The data collected from sensors will be delivered in different ways to Air quality server. In our model, Each sensor is an agent which has ability to opt for rational transmission line to send information packets. Basically, there are 3 types of transmission line:
\begin{enumerate}
\item Sensor $\rightarrow$ gNB $\rightarrow$ Air quality server.
\item Sensor $\rightarrow$ RSU $\rightarrow$ Air quality server.
\item Sensor A $\rightarrow$ Sensor B.
\end{enumerate}
The connection are depicted as below (specifically in the table \ref{tab:params}):
\begin{itemize}
\item Sensor $\rightarrow$ gNB: wireless connection, very slow speed.
\item Sensor $\rightarrow$ RSU: wireless connection, slow speed. 
\item Sensor A $\rightarrow$ Sensor B: wireless connection, slow speed.
\item gNB $\rightarrow$ Air quality server: wired connection, fast speed.
\item RSU $\rightarrow$ Air quality server: wired connection, fast speed.
\end{itemize}
Sensor is able to transfer information packets to another Sensor or RSU even when they are within each other's coverage. Every Sensor can always send information to the gNB. Our target is that each sensor will consecutively track the air quality along the roads and send the data collected to the Air quality server via 1 of 3 transmission ways listed above. However, transmission method of Sensor $\rightarrow$ 
gNB will be much more expensive. Therefore, the problem need to be solved is that How to minimize the number of packets are sending to the gNB and the necessary time for the packets to be delivered to the sever do not exceed the level $\delta$ specified previously.

The important symbols in this paper are listed in the following table:
\begin{table}[tb]
    \centering
    \caption{Notions \label{tab:notions}}
    \begin{tabular}{|m{1cm}|m{6.5cm}|}
    \hline
         \textbf{Notion} & \textbf{Description} \\
         \hline
         n & Number of Sensor \\
         m & Number of RSU \\
         $S$ & Sensor $S = \{S_1,...,S_i,...,S_n\}$ \\
         $r_{S_i}$ & Transmission radius of Sensor $i$ \\ 
         $C^*$ & Maximum capacity of Sensor\\
         $c_t$ & Capacity at state $t$ of Sensor \\
         $R$ & RSU $R = \{R_1,...,R_j,...,R_m\}$ \\ 
         $r_{R_j}$ & Transmission radius of RSU $j$ \\
         $\delta$ & Maximum time of the information packet \\
         $\mathcal{T}$ & Time slots $\mathcal{T} = \{1,...,t,...,T\}$ \\
         $\mathcal{S}$ & State space of the network\\
         $s_i(t)$ & State at a time $t$ of sensor $i$\\
         $\mathcal{A}$ & Action space of the network\\
         $a_i(t)$ & Action at a time $t$ of sensor $i$\\ 
         $\mu_t$ & Time to generate information packet \\
         $\Delta_t$ & Time since generating information packet to the time $t$\\
         $\theta$ & Parameter decide reward\\
         \hline
    \end{tabular}
\end{table}



\subsection{Q-learning}
\begin{figure}
    \centering
    \includegraphics[width=5cm]{figs/Q-learning.eps}
    \caption{Q-learning overview}
    \label{fig:q_learning}
\end{figure}

Q-Learning is a technique in Reinforcement Learning, learning through experiences to acquire specific optimization goal. Figure \ref{fig:q_learning} describes the overview model of Q-learning, including Environment, Agent, States and Action. Particularly, Q-learning is the algorithm We use to educate Q-function, an action-value function that determines the value of being at a certain state and taking a certain action at that state. Internally, our Q-function has a Q-table, which is a table where each cell corresponds to a state-action value pair value. And given a state and action, our Q-Function will search inside its Q-table to output the value. When the training is done, we have an optimal Q-function, so an optimal Q-Table. The Q value is updated according to the following equation:
\begin{equation}
Q(S_t, A_t) \leftarrow (1 - \alpha)Q(S_t, A_t) + \alpha[R_t + \gamma\max_{a}Q(S_{t+1}, a)]\label{eq}
\end{equation}
In which, $Q(S_t, A_t)$ is Q-value at a state $S_t$ when taking action $A_t$ at a time $t$. $R_t$ is the reward received for performing action $A_t$ in the state of $S_t$. $\max_{a}Q(S_{t+1}, a)$ is the maximum value of state $S_{t+1}$ for all possible action $a$. Furthermore, parameters $\alpha$ and $\gamma$ whose value is between $[0, 1]$ respectively is learning rate and discount rate. In our offer, each Sensor is considered to be an agent which has separate Q-table. Q-learning's mission is support agents to choose the right actions and achieve biggest reward. Detail information about rewards, state and action will be mentioned in part \ref{modeling_of_environment}.

 
\subsection{Fuzzy Logic}
\begin{figure}
    \centering
    \includegraphics[width=8.5cm]{figs/fuzzy-logic.eps}
    \caption{Fuzzy logic systems architecture}
    \label{fig:fuzzy_logic}
\end{figure}

The Fuzzy logic architecture depicted in figure \ref{fig:fuzzy_logic} consists of 4 main components: Fuzzification module, Knowledge base, Inference engine and Defuzzification module. 

% \begin{itemize}
    \subsubsection{Fuzzification module} it maps a real crisp input to a fuzzy function, therefore determining the "degree of membership ($\mu$)" of the input to a vague concept.
    \subsubsection{Knowledge base} it stores IF-THEN rules provided by experts. The expert knowledge is a collection of fuzzy membership functions and a set of fuzzy rules, known as the rule-base, having the form: \textbf{IF} (conditions are fulfilled) \textbf{THEN} (consequences are inferred). For more explicitly, a fuzzy rule with $k$-inputs and 1-output has the following form:
    \begin{equation}
    \begin{aligned}
        & \mathbf{IF} (I_1 \ \mathrm{is} \ A_{i1}) \Theta (I_2 \ \mathrm{is} \ A_{i2}) \Theta \cdots \Theta (I_k \ \mathrm{is} \ A_{ik}) \\
        & \mathbf{THEN} (O \ \mathrm{is} \ B_i)
    \end{aligned}
    \end{equation}
    where $\{I_1, \cdots ,I_k\}$ represents the crisp inputs to the rule. $\{A_{i1}, \cdots, A_{ik}\}$ and $B_i$ are linguistic variables. The operator $\Theta$ can be \textbf{AND}, \textbf{OR}, or \textbf{NOT}.
    \subsubsection{Inference engine} it deduces the fuzzy control actions by employing fuzzy implication and fuzzy rules of inference. It calculates the membership degree ($\mu$) of the output for all linguistic variables by applying the rule set. For Fuzzy rules with lots of inputs, the output calculation depends on the operators used inside it. The calculation for each type of operator is described as follows:
    % \begin{equation}
    % \begin{aligned}
    %     (I_i \ \mathrm{is} \ A_i \ & \mathbf{AND} \ I_j \ \mathrm{is} \  A_j): \\ 
    %     & \mu_{A_i \cap A_j} (I_{ij}) = \min (\mu_{A_i}(I_i), \mu_{A_j}(I_j))
    % \end{aligned}
    % \end{equation}
    % \begin{equation}
    % \begin{aligned}
    %     (I_i \ \mathrm{is} \ A_i \ & \mathbf{OR} \ I_j \ \mathrm{is} \  A_j): \\
    %     & \mu_{A_i \cup  A_j} (I_{ij}) = \max (\mu_{A_i}(I_i), \mu_{A_j}(I_j))
    % \end{aligned}
    % \end{equation}
    % \begin{equation}
    % \begin{aligned}
    %     (\mathbf{NOT} \ I_i \ \mathrm{is} \ A_i):& \\
    %     &\mu_{\bar{A_i}}(I_i) = 1 - \mu_{{A_i}}(I_i)
    % \end{aligned}
    % \end{equation}
    
    \begin{equation}
    \begin{aligned}
        (I_i \ \mathrm{is} \ A_i \ & \mathbf{AND} \ I_j \ \mathrm{is} \  A_j): \\ 
        & \mu_{A_i \cap A_j} (I_{ij}) = \min (\mu_{A_i}(I_i), \mu_{A_j}(I_j)) \\
        (I_i \ \mathrm{is} \ A_i \ & \mathbf{OR} \ I_j \ \mathrm{is} \  A_j): \\
        & \mu_{A_i \cup  A_j} (I_{ij}) = \max (\mu_{A_i}(I_i), \mu_{A_j}(I_j)) \\
        (\mathbf{NOT} \ I_i & \ \mathrm{is} \ A_i): \\
        &\mu_{\bar{A_i}}(I_i) = 1 - \mu_{{A_i}}(I_i) \\
    \end{aligned}
    \end{equation}
    
    \subsubsection{Defuzzification module} it process converts fuzzy control values into crisp quantities, that is, it links a single point to a fuzzy set, given that the point belongs to the support of the fuzzy set. There are many defuzzification techniques, the most famous being the centre-of-area (COA) or centre-of-gravity (COG). 
    % \\For discrete membership function, the defuzzified value denoted as $x^*$ using COG is defined as:
    % \begin{equation}
    %     x^{*} = \frac{\sum_{i=1}^{n}x_{i}.\mu (x_i)}{\sum_{i=1}^{n}\mu(x_i)}
    % \end{equation}
    % here $x_i$ indicates the sample element, $\mu(x_i)$ is the membership function, and $n$ represents the number of elements in the sample. 
    % \\For continuous membership function, $x^{*}$ is defined as:
    For continuous membership function, the defuzzified value denoted as $x^*$ using COG is defined as:
    \begin{equation}
    \label{eqn:fuzzy_defuzzification}
        x^{*} = \frac{\int x.\mu_A(x)dx}{\int \mu_A(x)dx} 
    \end{equation}
    where $\mu_A(x)$ is the output membership of the linguistic variable $A$.
% \end{itemize}



% Tiếng Việt ở đây 
% Các ký hiệu quan trọng trong bài báo này được liệt kê trong bảng sau:
% \begin{table}[ht!]
%     \centering
%     \caption{Notions \label{tab:notions}}
%     \begin{tabular}{|m{1cm}|m{6cm}|}
%     \hline
%          \textbf{Notion} & \textbf{Description} \\
%          \hline
%          n & Số lượng Sensor \\
%          m & Số lượng RSU \\
%          $S$ & Sensor $S = \{S_1,...,S_i,...,S_n\}$ \\
%          $r_{S_i}$ & Bán kính truyền tin của Sensor $i$ \\ 
%          $C^*$ & Dung lượng tối đa của Sensor\\
%          $c_t$ & Dung lượng tại thời điểm $t$ của Sensor \\
%          $R$ & RSU $R = \{R_1,...,R_j,...,R_m\}$ \\ 
%          $r_{R_j}$ & Bán kính truyền tin của RSU $j$ \\
%          $\delta$ & Thời gian tối đa cho phép của gói tin \\
%          $\mathcal{T}$ & Time slots $\mathcal{T} = \{1,...,t,...,T\}$ \\
%          $\mathcal{S}$ & Không gian trạng thái của mạng\\
%          $s_i(t)$ & Trạng thái tại thời điểm $t$ của sensor $i$\\
%          $\mathcal{A}$ & Không gian hành động của mạng\\
%          $a_i(t)$ & Hành động tại thời điểm $t$ của sensor $i$\\ 
%          $\mu_t$ & Thời gian sinh ra gói tin \\
%          $\Delta_t$ & Thời gian từ khi gói tin sinh ra đến thời điểm $t$\\
%          $\theta$ & Tham số quyết định phần thưởng\\
%          \hline
%     \end{tabular}
% \end{table}


% \subsection{Network Model} 
% \begin{figure}
%     \centering
%     \includegraphics[width=8cm]{figs/model.eps}
%     \caption{Network model}
%     \label{fig:network_model}
% \end{figure}

% Mô hình kiến trúc của chúng tôi được miêu tả trong hình \ref{fig:network_model}. Cụ thể, hệ thống của chúng tôi dựa trên mô hình MEC 3 tầng bao gồm: các thiết bị cảm biến đặt trên mỗi xe bus, các  đơn vị điện toán biên (RSU) và trung tâm xử lý đám mây (Cloud). Đầu tiên, về các thiết bị cảm biến, chúng tôi giả định rằng có $n$ sensor $S_i (i = 1,...,n)$ được đặt trên $n$ xe bus có tuyến đường cố định. Mỗi sensor có dung lượng tối đa là $C^*_i$ và bán kính truyền tin $r_{S_i}$. Thứ hai, có $m$  RSU $R_j (j = 1,...,m)$ có bán kính truyền tin $r_{R_j}$ được đặt cố định bên cạnh các tuyến đường. Thứ ba, 1 trung tâm đám mây có độ phủ sóng lớn tới mọi Sensor. Dữ liệu thu nhận được từ mỗi sensor sẽ được gửi thông qua các con đường khác nhau về Air quality server. Trong mô hình của chúng tôi, mỗi Sensor sẽ là một tác nhân có khả năng tự quyết định gửi gói tin theo các loại đường truyền sau:
% \begin{enumerate}
% \item Sensor $\rightarrow$ Cloud $\rightarrow$ Air quality server.
% \item Sensor $\rightarrow$ RSU $\rightarrow$ Air quality server.
% \item Sensor A $\rightarrow$ Sensor B.
% \end{enumerate}
% Các kết nối được miêu tả như sau (cụ thể trong bảng \ref{tab:params}):
% \begin{itemize}
% \item Sensor $\rightarrow$ Cloud: kết nối không dây, tốc độ rất chậm.
% \item Sensor $\rightarrow$ RSU: kết nối không dây, tốc độ chậm 
% \item Sensor A $\rightarrow$ Sensor B: kết nối không dây, tốc độ chậm.
% \item Cloud $\rightarrow$ Air quality server: kết nối có dây, tốc độ nhanh.
% \item RSU $\rightarrow$ Air quality server: kết nối có dây, tốc độ nhanh.
% \end{itemize}
% Sensor có thể truyền tin cho Sensor khác hay RSU khi cả 2 nằm trong vùng phủ sóng của nhau. Các Sensor luôn luôn có thể truyền tin lên Cloud. Mục tiêu của chúng tôi là các sensor sẽ theo dõi chất lượng không khí liên tục trên suốt đường đi và gửi thông tin về Air quality server theo 1 trong 3 con đường trên. Tuy nhiên, phương thức truyền tin từ Sensor $\rightarrow$ Cloud sẽ mất chi phí lớn. Chính vì vậy, vấn đề bài toán đặt ra nhằm tối thiểu dung lượng gói tin gửi về Cloud sao cho thời gian của các gói tin phải được gửi về server không quá ngưỡng $\delta$ quy định trước.


% \subsection{Q-learning}
% \begin{figure}
%     \centering
%     \includegraphics[width=5cm]{figs/Q-learning.eps}
%     \caption{Q-learning overview}
%     \label{fig:q_learning}
% \end{figure}

% Q-Learning là một kỹ thuật trong Reinforcement Learning, được học tập thông qua kinh nghiệm để đạt mục tiêu tối ưu cụ thể. Hình \ref{fig:q_learning} mô tả kiến trúc tổng quan của Q-learning, bao gồm Environment, Agent, States và Action. Cụ thể, Q-learning là thuật toán chúng tôi sử dụng để đào tạo Q-function, an action-value function that determines the value of being at a certain state and taking a certain action at that state. Internally, our Q-function has a Q-table, which is a table where each cell corresponds to a state-action value pair value. And given a state and action, our Q-Function will search inside its Q-table to output the value. When the training is done, we have an optimal Q-function, so an optimal Q-Table. The Q value is updated according to the following equation:
% \begin{equation}
% Q(S_t, A_t) \leftarrow (1 - \alpha)Q(S_t, A_t) + \alpha[R_t + \gamma\max_{a}Q(S_{t+1}, a)]\label{eq}
% \end{equation}
% Trong đó, $Q(S_t, A_t)$ là Q-value tại trạng thái $S_t$ khi thực hiện hành động $A_t$ vào thời điểm $t$. $R_t$ là phần thưởng nhận được khi thực hiện hành động $A_t$ trong trạng thái $S_t$. $\max_{a}Q(S_{t+1}, a)$ là giá trị cực đại của trạng thái $S_{t+1}$ cho tất cả các hành động có thể $a$. Hơn nữa, tham số $\alpha$ và $\gamma$ có giá trị nằm trong khoảng $[0, 1]$ lần lượt là learning rate và discount rate. Trong đề xuất của chúng tôi, mỗi Sensor sẽ được coi là agent có Q-table riêng biệt. Nhiệm vụ của Q-learning sẽ giúp cho các tác nhân có thể lựa chọn hành động đạt được phần thưởng lớn nhất. Cụ thể chi tiết về phần thưởng, trạng thái và hành động sẽ được đề cập trong phần \ref{modeling_of_environment}.

 
% \subsection{Fuzzy Logic}
% \begin{figure}
%     \centering
%     \includegraphics[width=8.5cm]{figs/fuzzy-logic.eps}
%     \caption{Fuzzy logic systems architecture}
%     \label{fig:fuzzy_logic}
% \end{figure}

% The Fuzzy logic architecture depicted in figure \ref{fig:fuzzy_logic} consists of 4 main components: Fuzzification module, Knowledge base, Inference engine and Defuzzification module. 

% % \begin{itemize}
%     \subsubsection{Fuzzification module} it maps a real crisp input to a fuzzy function, therefore determining the "degree of membership ($\mu$)" of the input to a vague concept.
%     \subsubsection{Knowledge base} it stores IF-THEN rules provided by experts. The expert knowledge is a collection of fuzzy membership functions and a set of fuzzy rules, known as the rule-base, having the form: \textbf{IF} (conditions are fulfilled) \textbf{THEN} (consequences are inferred). For more explicitly, a fuzzy rule with $k$-inputs and 1-output has the following form:
%     \begin{equation}
%     \begin{aligned}
%         & \mathbf{IF} (I_1 \ \mathrm{is} \ A_{i1}) \Theta (I_2 \ \mathrm{is} \ A_{i2}) \Theta \cdots \Theta (I_k \ \mathrm{is} \ A_{ik}) \\
%         & \mathbf{THEN} (O \ \mathrm{is} \ B_i)
%     \end{aligned}
%     \end{equation}
%     where $\{I_1, \cdots ,I_k\}$ represents the crisp inputs to the rule. $\{A_{i1}, \cdots, A_{ik}\}$ and $B_i$ are linguistic variables. The operator $\Theta$ can be \textbf{AND}, \textbf{OR}, or \textbf{NOT}.
%     \subsubsection{Inference engine} it deduces the fuzzy control actions by employing fuzzy implication and fuzzy rules of inference. It calculates the membership degree ($\mu$) of the output for all linguistic variables by applying the rule set. For Fuzzy rules with lots of inputs, the output calculation depends on the operators used inside it. The calculation for each type of operator is described as follows:
%     % \begin{equation}
%     % \begin{aligned}
%     %     (I_i \ \mathrm{is} \ A_i \ & \mathbf{AND} \ I_j \ \mathrm{is} \  A_j): \\ 
%     %     & \mu_{A_i \cap A_j} (I_{ij}) = \min (\mu_{A_i}(I_i), \mu_{A_j}(I_j))
%     % \end{aligned}
%     % \end{equation}
%     % \begin{equation}
%     % \begin{aligned}
%     %     (I_i \ \mathrm{is} \ A_i \ & \mathbf{OR} \ I_j \ \mathrm{is} \  A_j): \\
%     %     & \mu_{A_i \cup  A_j} (I_{ij}) = \max (\mu_{A_i}(I_i), \mu_{A_j}(I_j))
%     % \end{aligned}
%     % \end{equation}
%     % \begin{equation}
%     % \begin{aligned}
%     %     (\mathbf{NOT} \ I_i \ \mathrm{is} \ A_i):& \\
%     %     &\mu_{\bar{A_i}}(I_i) = 1 - \mu_{{A_i}}(I_i)
%     % \end{aligned}
%     % \end{equation}
    
%     \begin{equation}
%     \begin{aligned}
%         (I_i \ \mathrm{is} \ A_i \ & \mathbf{AND} \ I_j \ \mathrm{is} \  A_j): \\ 
%         & \mu_{A_i \cap A_j} (I_{ij}) = \min (\mu_{A_i}(I_i), \mu_{A_j}(I_j)) \\
%         (I_i \ \mathrm{is} \ A_i \ & \mathbf{OR} \ I_j \ \mathrm{is} \  A_j): \\
%         & \mu_{A_i \cup  A_j} (I_{ij}) = \max (\mu_{A_i}(I_i), \mu_{A_j}(I_j)) \\
%         (\mathbf{NOT} \ I_i & \ \mathrm{is} \ A_i): \\
%         &\mu_{\bar{A_i}}(I_i) = 1 - \mu_{{A_i}}(I_i) \\
%     \end{aligned}
%     \end{equation}
    
%     \subsubsection{Defuzzification module} it process converts fuzzy control values into crisp quantities, that is, it links a single point to a fuzzy set, given that the point belongs to the support of the fuzzy set. There are many defuzzification techniques, the most famous being the centre-of-area (COA) or centre-of-gravity (COG). 
%     % \\For discrete membership function, the defuzzified value denoted as $x^*$ using COG is defined as:
%     % \begin{equation}
%     %     x^{*} = \frac{\sum_{i=1}^{n}x_{i}.\mu (x_i)}{\sum_{i=1}^{n}\mu(x_i)}
%     % \end{equation}
%     % here $x_i$ indicates the sample element, $\mu(x_i)$ is the membership function, and $n$ represents the number of elements in the sample. 
%     % \\For continuous membership function, $x^{*}$ is defined as:
%     For continuous membership function, the defuzzified value denoted as $x^*$ using COG is defined as:
%     \begin{equation}
%     \label{eqn:fuzzy_defuzzification}
%         x^{*} = \frac{\int x.\mu_A(x)dx}{\int \mu_A(x)dx} 
%     \end{equation}
%     where $\mu_A(x)$ is the output membership of the linguistic variable $A$.
% % \end{itemize}



